The Limitations of Stylometry for Detecting Machine-Generated Fake News

Recent developments in neural language models (LMs) have raised concerns about their potential misuse for automatically spreading misinformation. In light of these concerns, several studies have proposed to detect machine-generated fake news by capturing their stylistic differences from human-written text. These approaches, broadly termed stylometry, have found success in source attribution and misinformation detection in human-written texts. However, in this work, we show that stylometry is limited against machine-generated misinformation. While humans speak differently when trying to deceive, LMs generate stylistically consistent text, regardless of underlying motive. Thus, though stylometry can successfully prevent impersonation by identifying text provenance, it fails to distinguish legitimate LM applications from those that introduce false information. We create two benchmarks demonstrating the stylistic similarity between malicious and legitimate uses of LMs, employed in auto-completion and editing-assistance settings. Our findings highlight the need for non-stylometry approaches in detecting machine-generated misinformation, and open up the discussion on the desired evaluation benchmarks.

==> sections/realted-long.tex <==
\section{Background}

%prevent impersonations~\citep{Tweedie1996NeuralNA, brennan2012adversarial, Afroz2014DoppelgngerFT, anon15usenix, Neal2017SurveyingST}; (2) \textit{Detecting misinformation} in text due to deception~\citep{Mihalcea2009TheLD, Ott2011FindingDO, Feng2012stylometry, Afroz2012DetectingHF}, fake news~\citep{rashkin2017truth, perez2017automatic}, or other false or illegal content~\citep{Choshen2019TheLO}. 

\paragraph{Stylometry for Human-written Text} 
The use of statistical methods for analyzing human-written documents has been studied extensively since the early days of the field. \citet{authorship1963} used word counts to predict the authorship of historical documents. \citet{Tweedie1996NeuralNA} applied a neural network to the same task, considering a wider range of stylistic features. \citet{brennan2012adversarial} have shown that authorship classifiers can be fooled by writers that intentionally alternate their style and imitate another subject. Recent studies explored stylometry tools on even more challenging tasks such as de-anonymizing cybercriminals in underground forums~\citep{Afroz2014DoppelgngerFT} and identifying programmers via analyzing source code~\citep{anon15usenix}. We refer the reader to~\citet{Neal2017SurveyingST} for a more comprehensive survey.

The collection of new datasets over the last several years allowed researchers to extend the study of stylometry beyond author identification. In one line of study, stylometry methods were applied to identify  characteristics of the author, such as age and gender~\citep{goswami2009stylometric}, political views~\citep{potthast-etal-2018-stylometric}, or IQ level~\citep{abramov2019automatic}.
The applications of stylometry that are most relevant to this paper are the ones that aim to identify changes in the writing style of the same author. \citet{Mihalcea2009TheLD} asked people to write true and false statements and identified words that highly correlate with each class. \citet{Ott2011FindingDO, Feng2012stylometry} used a reacher set of features such as POS tags frequencies and constituency structure. They also found correlation between deceptive and imaginative writing in humans.

Recently, the increasing interest in fake news detection has motivated studies to apply stylometry on entire news articles~\citep{pisarevskaya-2017-deception}, short news reports~\citep{perez2017automatic}, fact and political statements~\citep{nakashole-mitchell-2014-language, rashkin2017truth} and posts in social media~\citep{volkova-etal-2017-separating}. The success of these studies is mostly attributed to stylistic changes in human language when lying or deceiving~\citep{bond2005prison,frank2008human}.
%In this work, we create benchmarks with machine-generated false information, thus reducing the stylistic differences between truth and lie.
In this work, we evaluate the viability of this approach on machine-generated text, where stylistic differences between truth and lie might be more subtle.

\paragraph{Machine-generated Text Detection}% \ \\
%The recent improvement in the quality of text generated by language models (LM) motivated several studies to examine their differences from human-written text.
Detecting text's provenance is similar to authorship attribution and, therefore, stylometry can be effective. Indeed, \citet{gehrmann2019gltr} show the existence of distributional differences between human-written texts and machine-generated ones by visualizing the per-token probability according to a LM.
\citet{bakhtin2019real} learn a dedicated provenance neural classifier. While their classifier achieves high in-domain accuracy, they find that it overfits the generated text distribution rather than detecting outliers from human texts, resulting in increased ``human-ness'' scores for random perturbations.
Nevertheless, an advantage of such neural approaches over more traditional stylometry is that, given enough data, the model learns hidden stylistic representations without the need to manually define any features. 

% Building on the above observation, \citet{zellers2019defending} focus on fake news and create a model dubbed Grover. This model can both generate news articles and detect auto-generated news based on provenance. 
Building on the above observation, \citet{zellers2019defending} focus on fake news and create a Transformer-based LM~\citep{vaswani2017attention} dubbed Grover and train it on a large news corpus.
Grover also includes a ``fake news detector'', a linear classifier on top of the hidden state of the last token of the examined article, fine-tuned on the classification task. Despite its stated designation, Grover does not detect fake news per se; rather, it is a powerful provenance-based detector for machine-generated text.
%Grover's fake news \textit{detector} is a linear classifier on top of the last the LM on the examined article, fine-tuned on the classification task.



% \paragraph{Grover's Architecture} \label{attackmodel}%\ \\
% Grover's news \textit{generator} is a Transformer-based LM~\citep{vaswani2017attention}. Though architecturally similar to GPT-2~\citep{radford2019language}, the generator was trained specifically on news article texts, conditioned on the article meta-data, and its output tokens are sampled using nucleus sampling~\citep{holtzman2019curious}. The generator is trained with a LM objective on a large news corpus from Common Crawl dumps.

% The fake news \textit{detector} is a linear classifier on top of the last hidden state of Grover's LM on the examined article. The LM parameters are initialized with the pre-trained generator values, from an earlier checkpoint, and are optimized jointly with the linear layer on the classification training set. To construct this dataset, fake news were generated by the pretrained generator and real news were sampled human-written articles.
% \tal{maybe merge this with prev parag. to save space}









% \paragraph{Rumor Propagation} 
% Assessing the reliability of information propagated in social networks has recently been of high interest. To this end, methods that leverage features of the content's propagation pattern~\citep{castillo2011information, gupta2014tweetcred, liu2015real, nguyen2019fake, ma2018detect, ma2016detecting, kochkina2018all, liu2018early,  zhao2015enquiring}, patterns of reaction to content~\cite{gupta2014tweetcred, liu2018early, nguyen2019fake,  ma2018detect, zhao2015enquiring, kochkina2018all, castillo2011information}, characteristics of the propagating users~\cite{gupta2014tweetcred, nguyen2019fake, liu2018early, castillo2011information, popat2016credibility}, and, finally, features of the textual content itself~\cite{gupta2014tweetcred, popat2016credibility} were applied. This line of work focuses on detecting fake news or rumors focused on settings where ample auxiliary information exists, beyond the potentially disputable text itself.

% \paragraph{Fake News Propagation Detection}
% An extensive line of work~\citep{castillo2011information, gupta2014tweetcred, liu2015real, nguyen2019fake, ma2018detect, ma2016detecting, kochkina2018all, liu2018early,  zhao2015enquiring} focuses on detecting disinformative content by examining how, and by whom, it is propagated within a social network. In this attack setting, ample auxiliary information exists beyond the potentially disputable text.
